Distributed Quantum Faithful Simulation and Function Computation Using Algebraic Structured Measurements

In this work, we consider the task of faithfully simulating a quantum measurement, acting on a joint bipartite quantum state, in a distributed manner. In the distributed setup, the constituent sub-systems of the joint quantum state are measured by two agents, Alice and Bob. A third agent, Charlie receives the measurement outcomes sent by Alice and Bob. Charlie uses local and pairwise shared randomness to compute a bivariate function of the measurement outcomes. The objective of three agents is to faithfully simulate the given distributed quantum measurement acting on the given quantum state while minimizing the communication and shared randomness rates. We demonstrate a new achievable information-theoretic rate-region that exploits the bivariate function using random structured POVMs based on asymptotically good algebraic codes. The algebraic structure of these codes is matched to that of the bivariate function that models the action of Charlie. The conventional approach for this class of problems has been to reconstruct individual measurement outcomes corresponding to Alice and Bob, at Charlie, and then compute the bivariate function, achieved using mutually independent approximating POVMs based on random unstructured codes. In the present approach, using algebraic structured POVMs, the computation is performed on the fly, thus obviating the need to reconstruct individual measurement outcomes at Charlie. Using this, we show that a strictly larger rate region can be achieved. One of the challenges in analyzing these structured POVMs is that they exhibit only pairwise independence and induce only uniform single-letter distributions. To address this, we use nesting of algebraic codes and develop a covering lemma applicable to pairwise-independent POVM ensembles. Combining these techniques, we provide a multi-party distributed faithful simulation and function computation protocol.

==> abstract.tex <==
\begin{abstract}
  In this work, we consider the task of faithfully simulating a distributed quantum measurement  and demonstrate a new achievable information-theoretic rate-region. We accomplish this  by developing a technique of randomly generating structured POVMs using algebraic codes. One of the major challenges toward employing these structured POVMs is that they only exhibit pairwise independence. To overcome this
%   we develop a Pruning Trace inequality which is a tighter version of the known operator Markov inequality. In addition, 
we develop a covering lemma, independent of the operator Chernoff inequality, and applicable to pairwise-independent operators.
 We demonstrate rate gains for this problem and also for the problem of distributed function computation over traditional coding schemes. 
 Combining these techniques, we provide a multi-party distributed faithful simulation and function computation protocol.  
\end{abstract}

% and function computation,
